Gravitational lensing of pulsars as a probe of dark matter halos

An open question in cosmology is whether dark matter forms gravitationally bound halos on small scales within the Galaxy. Since gravitational lensing probes matter independently of its microscopic composition, it offers a means of investigating such structures without assuming a particular dark matter candidate. This thesis develops a relativistic and numerical framework for investigating the gravitational-lensing signatures of low-mass dark matter halos in millisecond pulsar observations. The method calculates image positions, magnifications and propagation delays for individual lenses, transforms their signatures into the observer's frame, and extends the simulations to exploratory populations of independently transiting halos. Several lens models are considered, including the Navarro--Frenk--White density profile, while Hankel transforms improve the efficiency of evaluating axisymmetric lensing potentials. The simulations demonstrate time-dependent timing and amplitude signatures that could motivate searches for Galactic dark matter substructure using the rotational stability of millisecond pulsars. The thesis also examines the limitations of idealised halo populations, numerical approximations and the recovery of lensing signatures from observational timing data.

==> chapter2/ltfile.tex <==
% \loadgeometry{widetable-layout}

% Reactions in box that can be used in tabular
\newsavebox{\mybox}
\sbox{\mybox}{
\begin{minipage}{0.45\linewidth}
\begin{align*}
\begin{aligned}
 p + n &\rightarrow d + \gamma \;
\end{aligned} &\text{fusion of deuterium} \\
\left.\begin{aligned}
d + p &\rightarrow \text{$^3$He} + \gamma \\
d + d &\rightarrow \text{$^3$He} + n \\
d + d &\rightarrow t + p \\
\text{$^3$He} + n &\rightarrow t + p \\
\end{aligned}
\;\right\}\;
&\text{\begin{minipage}{3.2cm}production of $^3$He \\ and tritium $t$ \end{minipage}} 
\\
\left.\begin{aligned}
\text{$^3$He} + d &\rightarrow \text{$^4$He} + p \\
t + d &\rightarrow \text{$^4$He} + n \\
\end{aligned}
\;\right\}\;
&\text{conversion to $^4$He} \\
\left.\begin{aligned}
t + \text{$^4$He} &\rightarrow \text{$^7$Li} + \gamma \\
\text{$^3$He} + \text{$^4$He} &\rightarrow \text{$^7$Be} + \gamma \\
\text{$^7$Be} + e^- &\rightarrow \text{$^7$Li} + \nu_e \\
\end{aligned}
\;\right\}\;
&\text{Lithium production}
\end{align*}
\end{minipage}
}
% End of savebox


\begin{figure}
%%----start of first figure graphics----
\begin{minipage}{0.48\linewidth}
\centering
\includegraphics[width=\textwidth]{bbn-abundances} 
\end{minipage}%
\hspace{.5cm}%
%%----start of second figure graphics----
\begin{minipage}{0.48\linewidth}
\centering
\begin{longtable}{p{0.5\linewidth} l} % first col = width of eqns
\\[-45pt]
\toprule % begin header
Reaction & Element production \\
\midrule  \\[-.25in]
\endfirsthead % end of header
\bottomrule
\endlastfoot % end footer
% standard tabular environment content
\multicolumn{2}{c}{\usebox{\mybox}} \\
\bottomrule
% standard tabular environment ends
\end{longtable}
\end{minipage}
\\%[-10pt]
%%----start of first figure caption----
\begin{minipage}[t]{.5\linewidth}
\captionof{figure}{Theoretically expected abundances (relative to hydrogen) of the light elements deuterium ($D$), helium ($^{3}$He and $Y = ^{4}$He) and lithium($^{7}$Li) as functions of the abundance ratio $\eta_{10}$. The widths of each band are caused by the uncertainties in the nuclear and weak-interaction rates. (Fig.~5 in \cite{bbn-summary}) \label{fig:bbn}}
\end{minipage}%
%\hspace{1cm}%
%%----start of second figure caption----
\begin{minipage}[t]{.5\linewidth}
\captionof{table}{Reactions involved in primordial neucleosynthesis.  \label{tab:bbn}} 
\end{minipage}%
\end{figure}
% \restoregeometry

==> chapter2/parameter-space-horiz.tex <==
\begin{figure}[bh]
%%----start of first figure graphics----
\begin{minipage}{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{sterile} 
\end{minipage}%
%\hspace{.5cm}%
%%----start of second figure graphics----
\begin{minipage}{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{axions} 
\end{minipage}
\\%[-10pt]
%%----start of first figure caption----
\begin{minipage}[t]{.5\linewidth}
\captionof{figure}{Parameter space for the sterile neutrino mass $m_{\nu}$ and mixing angle $\theta$.  Regions which are yellow are \textit{favoured} by astrophysical observations (darker regions have higher likelihood).  Regions shaded in other colours are \textit{excluded} by their respective observations while the red region is excluded on theoretical grounds. (Fig.~20 in \cite{dm-particles}) \label{fig:sterile}}
\end{minipage}%
%\hspace{1cm}%
%%----start of second figure caption----
\begin{minipage}[t]{.5\linewidth}
\captionof{figure}{Credible regions for the axion parameters $g_{\ast}$ (thermal degrees of freedom) and $\Omega_a$ (cosmological density) from cosmological sources.  The axion mass in eV is indicated by the dashed lines.  Regions which are unshaded are \textit{excluded} at the 95\% CL; regions which are lightly shaded are also excluded at the 68\% CL.  (Fig.~5 in \cite{axions}) \label{fig:axions}} 
\end{minipage}%
\end{figure}
